Autoformalize Mathematical Statements by Symbolic Equivalence and Semantic Consistency

Autoformalization, the task of automatically translating natural language descriptions into a formal language, poses a significant challenge across various domains, especially in mathematics. Recent advancements in large language models (LLMs) have unveiled their promising capabilities to formalize even competition-level math problems. However, we observe a considerable discrepancy between pass@1 and pass@k accuracies in LLM-generated formalizations. To address this gap, we introduce a novel framework that scores and selects the best result from k autoformalization candidates based on two complementary self-consistency methods: symbolic equivalence and semantic consistency. Elaborately, symbolic equivalence identifies the logical homogeneity among autoformalization candidates using automated theorem provers, and semantic consistency evaluates the preservation of the original meaning by informalizing the candidates and computing the similarity between the embeddings of the original and informalized texts. Our extensive experiments on the MATH and miniF2F datasets demonstrate that our approach significantly enhances autoformalization accuracy, achieving up to 0.22-1.35x relative improvements across various LLMs and baseline methods.

==> 005_tbd.tex <==
\section{Related Work}\label{sec:relate}

Let us start with the majority voting in code generation. % first rethink
The efficacy of the approach fundamentally relies on the \emph{assumption} that correct programs are logically equivalent, whereas incorrect ones are likely not~\citep{chen2022codet, huang2023enhancing, li2022competition}. 
This implies that correct programs yield identical outputs for the same input, while incorrect ones produce varying results.
Adopting this principle and bypassing the concrete execution used in code generation leads to a symbolic majority voting strategy: if two autoformalized statements are logically equivalent, they should be assigned to a same class. 
Then, we can just select a formal statement in the majority class as the final result. 

% \begin{enumerate}
%     \item the background of theorem proving.
%     \item the use of LLM for autoformalization. One of the key is to define autoformalization as $Statement_{NL} \rightarrow (p \Rightarrow q)$
% \end{enumerate}

%  The research of autoformalization spans the entire evolution of artificial intelligence~\citep{mc1969some, simon1988checking, szegedy2020promising}, 
but the progress is still modest.

\subsection{Formal Mathematics}  
The goal of formal mathematics is to provide a rigorous framework for expressing and verifying mathematical truths, so that mathematical reasoning can be checked by a computer ``program'' following logical rules instead of a ``small group of people''. In recent years, with the development of {\em interactive theorem provers} (e.g., Isabelle/HOL \cite{paulson1994isabelle}, Lean \cite{de2015lean}, Coq \cite{bertot2013interactive}), some challenging mathematical theorems and concepts \cite{gonthier2008four,gonthier2013machine,hales2017formal,buzzard2020formalising,scholze2022liquid} have been manually formalized and verified to be correct, demonstrating the power and the potential of formal mathematics.

However, formalizing mathematical statements and proofs into a language that theorem provers can interpret is a non-trivial task, which often requires a deep understanding of both the mathematics involved and the syntax of the target formal language. Therefore, the formalization process is often time-consuming even with large groups of experts, which hinders the development of formal mathematics. \zhaoyu{shall we add some citations? Gödel’s Incompleteness Theorems,Formal Abstracts,mathlib}
% Theorem proving is a critical aspect of mathematical verification, where the goal is to formally prove or disprove that certain statements or proofs according to a {\bf program} following logical rules. This program, often called as theorem prover, is categorized as twofold:
% \begin{itemize}
% \item Automatic theorem prover (ATP), which is an automated program to prove statements without human intervention once the statement is formalized as low-level solver problems such as Boolean satisfiability (SAT) problems or satisfiability modulo theories (SMT) problems \cite{de2008z3,barrett2011cvc4}.
% \item Interactive theorem prover, which is a semi-automated program that requires human interactions to complete a proof when the proof is non-trivial for ATP \cite{paulson1994isabelle, de2015lean, bertot2013interactive}.  
% \end{itemize}  



\subsection{Autoformalization with Large Language Models}  

{We should claim that this is a method without fine-tuning.}

Large language models (LLM) have recently been used to automate the process of formalizing mathematical statements and proofs, a process we refer to as statement autoformalization \cite{wu2022autoformalization,wang2018first,liu2023fimo} and proof autoformalization \cite{jiang2022draft,wang2023legoprover}, respectively. In statement autoformalization, translation pairs are often provided as prompt examples to guide the LLM formalizations \cite{wu2022autoformalization}. By contrast, the proof autoformalization process is more challenging and complicated, which requires the LLM to first draft natural language proof, sketch the proof structure, and then elaborate the proof with an automated search using specific tactics (e.g., $\mathtt{ sledgehammer, auto}$ in Isabelle/HOL) \cite{jiang2022draft}.

In this work, we focus on statement autoformalization but also leverage automated search techniques in proving symbolic equivalence. We mainly explore the potential of existing LLMs for autoformalization without the additional process of retrieval or fine-tuning, which may potentially boost the autoformalization accuracy of top10 predictions. We leave them for future work.

% These models take a statement in natural language ($Statement_{NL}$) and attempt to translate it into a formal representation typically expressed as an implication ($p \Rightarrow q$), where $p$ represents the premises and $q$ represents the conclusion. The successful application of LLMs to autoformalization suggests that they can learn and replicate the complex patterns of formal mathematical language, offering a promising tool for scaling up the formalization process in theorem proving.  

% \subsection{Majority Voting with LLM Outputs}  
% LLMs suffer from the ``hallucination problem'', which means that they often generate buggy outputs with factual errors or reasoning flaws \cite{?}. To mitigate this problem, one of the most conventional approaches is to use majority voting to select the most frequent output from multiple runs of the LLM \cite{wang2022self,,,}. For example, \citet{wang2022self} introduces {\em self-consistency} technique to prompt LLMs for multiple chain-of-thought outputs and select the most frequent answer as the final reasoning output.

% However, for the task of autoformalization, the traditional majority voting approach is not applicable because the LLM formalizations are often diverse and not directly comparable. Formalizations which are apparently different may be symbolically equivalent and semantically consistent, which inspire us to use the novel majority voting to select the most promising formalization from the maximum cluster.
\subsection{AI Math Reasoning}
While LLMs like GPT-4 have achieved tremendous progress in the conversation and language understanding tasks \cite{achiam2023gpt}, they are still far from being able to perform complex mathematical reasoning. For example, current GPT-4 can solve 52\% problems in the MATH dataset \cite{hendrycks2021measuring}, which is much lower than the expert performance ($\sim 90\%$). To address this problem, prior work propose to leverage symbolic tools such as interactive theorem provers \cite{anonymous2024dont} and SymPy \cite{zhou2023solving, gou2023tora} to boost the math performance of LLMs. All these work rely on the translation from natural language to symbolic language, which are similar to the process of autoformalization. 


\subsection{Code Verification and Generation}
% \xian{is this subsection necessary?}
Formal mathematics is highly related to the formal verification of code, where properties of the code or so so-called specification are proved through the process of theorem proving. For example, the seL4 project leverages the Isabelle theorem prover to formally verify the specification of a microkernel \cite{klein2009sel4}. With the specification, high-performance C code is implemented accordingly. And it took tens of experts many years to formalize the specification and prove the properties, which may be largely accelerated with techniques of autoformalization and automatic theorem proving.

The autoformalization process is also related to the code generation of LLMs, where the goal is to generate code from natural language descriptions and the majority voting techniques are widely considered ~\citep{chen2022codet, huang2023enhancing, li2022competition}. However, for the task of autoformalization, the traditional majority voting approach is not applicable because the LLM formalizations are often diverse and not directly comparable. Formalizations that are apparently different may be symbolically equivalent and semantically consistent, which inspires us to use the novel majority voting to select the most promising formalization from the maximum cluster.

==> deleted.tex <==
% To address these challenges, we propose a novel framework that establishes the self-consistency of autoformalization from two different aspects. In this framework, we first generalize the comparison of reasoning answers and execution behaviors to \emph{symbolic equivalence} among autoformalization candidates. Symbolic equivalence can be verified through existing automated theorem provers (e.g., sledgehammer~\citep{bohme2010sledgehammer}, Z3~\citep{de2008z3}, and CVC5~\citep{barbosa2022cvc5}). 
% Next, we introduce \emph{semantic consistency} to alleviate the unintended reasoning issue of the symbolic equivalence. 
% Semantic consistency measures the autoformalization error by comparing the re-informalized (i.e., back-translated~\citep{edunov2018understanding}) result and the original statement.
% Finally, we design three combination strategies on the scores derived from these two methods. 
% Meanwhile, semantic consistency addresses unintended reasoning discrepancies by comparing the re-informalized (back-translated \citep{edunov2018understanding}) result with the original statement. 
% \citet{wu2022autoformalization} studies LLMs with few-shot prompting to translate mathematical problems at the high school level into Isabelle.

% To faithfully evaluate the equivalence between two mathematical statements, we propose a novel hybrid strategy that incorporates both symbolic and semantic information of mathematics. 
% To faithfully identify the homogeneity among autoformalized theorems, 
% we propose a novel hybrid framework \framework{} that incorporates both symbolic and semantic information of mathematics. 
% Elaborately, \framework{} achieves 

% we compute two scores from two aspects: (1) symbolic equivalence and (2) semantic consistency, respectively.  Then, we derive a final score for the autoformalization by a weighted combination of these two scores. 


% In summary, for the selection from autoformalization candidates, three point still impede its success: (1) The limited capability of ATPs; (2) The shortcuts issue of LLMs; (3) The lack of voting strategy. 


% Then, the symbolic equivalence between two statements can be defined as the two logical equivalences between their premises and their conclusions.

% It is also worth noting that the validity of the premises can be checked by the prover. 
% Specifically, one can simply replace the conclusion $\mathcal{Q}$ by any contradictory result (e.g., $0 = 1$), and using the automated theorem prover to verify $\mathcal{P} \to \mathcal{Q}$.


% The merit of this framework lies in a complementary combination
% of symbolic equivalence and semantic consistency, 
% in which
% symbolic equivalence identifies the logical homogeneity among autoformalization candidates, while semantic consistency ensures coherence with the original natural language statement. 

(e.g., relative improvements of 7.57\%-10.25\% for GPT-4) over existing baselines and alternatives. 
Achieve relative efficency compared to the baseline  xxxx\%
